A Unification Algorithm for GP 2 (Long Version)

The graph programming language GP 2 allows to apply sets of rule schemata (or "attributed" rules) non-deterministically. To analyse conflicts of programs statically, graphs labelled with expressions are overlayed to construct critical pairs of rule applications. Each overlay induces a system of equations whose solutions represent different conflicts. We present a rule-based unification algorithm for GP expressions that is terminating, sound and complete. For every input equation, the algorithm generates a finite set of substitutions. Soundness means that each of these substitutions solves the input equation. Since GP labels are lists constructed by concatenation, unification modulo associativity and unit law is required. This problem, which is also known as word unification, is infinitary in general but becomes finitary due to GP's rule schema syntax and the assumption that rule schemata are left-linear. Our unification algorithm is complete in that every solution of an input equation is an instance of some substitution in the generated set.

==> graphs_config.tex <==
% Local configuration for version 1.53 of graphs.sty. Frank Drewes, 16.11 2003

% The \special macro below must contain the path under which the file
% graphs.header can be found in you local installation. Please modify it
% accordingly.

\special{header=graphs.header}


==> graphs_ps.tex <==
% `special' commands for version 1.53 of graphs.sty. Frank Drewes, 16/11 2003

\def\ps@s{ }
\def\ps@convertnum#1{
	#1 \number\unitlength\ps@s mul 65536 div 72.27 div 72 mul
}

%-----------------------------------------------------------------------------%


\def\ps@rectangle[#1,#2]{% width, height
\special{"	\ps@convertnum{#1}
		\ps@convertnum{#2}
		[ \g@ncolour\ps@s\g@ncolourmod ]\ps@s
		[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
		\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
		\g@ldash\ps@s
		\iffillednodes true \else false\fi\ps@s
		psrectangle}}

%-----------------------------------------------------------------------------%

\def\ps@circle[#1]{% diameter
\special{"	\ps@convertnum{#1}
		[ \g@ncolour\ps@s\g@ncolourmod ]\ps@s
		[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
		\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
		\g@ldash\ps@s
		\iffillednodes true \else false\fi\ps@s
		pscircle}}

%-----------------------------------------------------------------------------%

\def\ps@line(#1,#2){% end x, end y
\special{"	\ps@convertnum{#1}
		\ps@convertnum{#2}
		\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
		[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
		\g@ldash\ps@s
		psline}}

%-----------------------------------------------------------------------------%

\def\ps@loopA(#1,#2)(#3,#4){% from (#1,#2) to (#3,#4)
\special{"	\ps@convertnum{#1}
		\ps@convertnum{#2}
		\ps@convertnum{#3}
		\ps@convertnum{#4}
		[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
		\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
		\g@ldash\ps@s
		psloop}}

%-----------------------------------------------------------------------------%

\def\ps@loopB#1(#2,#3){% angle #1, axis (#2,#3)
\special{"	#1
		\ps@convertnum{#2}
		\ps@convertnum{#3}
		psloopbyangle
		[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
		\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
		\g@ldash\ps@s
		psloop}}
		
%-----------------------------------------------------------------------------%

\def\ps@looparrowonrectangleA(#1,#2)(#3,#4)[#5,#6]{% 
\special{"	\ps@convertnum{#1}
		\ps@convertnum{#2}
		\ps@convertnum{#3}
		\ps@convertnum{#4}
		\ps@convertnum{#5}
		\ps@convertnum{#6}
		[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
		\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
		\g@ldash\ps@s
		\ps@convertnum{\g@alength}\g@alengthmod\ps@s
		\g@awidth\ps@s\g@awidthmod\ps@s
		\g@atype\ps@s
		pslooparrowonrectangle}}

%-----------------------------------------------------------------------------%

\def\ps@looparrowoncircleA(#1,#2)(#3,#4)[#5]{% 
\special{"	\ps@convertnum{#1}
		\ps@convertnum{#2}
		\ps@convertnum{#3}
		\ps@convertnum{#4}
		\ps@convertnum{#5}
		[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
		\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
		\g@ldash\ps@s
		\ps@convertnum{\g@alength}\g@alengthmod\ps@s
		\g@awidth\ps@s\g@awidthmod\ps@s
		\g@atype\ps@s
		pslooparrowoncircle}}

%-----------------------------------------------------------------------------%

\def\ps@looparrowonrectangleB#1(#2,#3)[#4,#5]{% 
\special{"	#1
		\ps@convertnum{#2}
		\ps@convertnum{#3}
		psloopbyangle
		\ps@convertnum{#4}
		\ps@convertnum{#5}
		[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
		\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
		\g@ldash\ps@s
		\ps@convertnum{\g@alength}\g@alengthmod\ps@s
		\g@awidth\ps@s\g@awidthmod\ps@s
		\g@atype\ps@s
		pslooparrowonrectangle}}

%-----------------------------------------------------------------------------%

\def\ps@looparrowoncircleB#1(#2,#3)[#4]{% 
\special{"	#1
		\ps@convertnum{#2}
		\ps@convertnum{#3}
		psloopbyangle
		\ps@convertnum{#4}
		[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
		\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
		\g@ldash\ps@s
		\ps@convertnum{\g@alength}\g@alengthmod\ps@s
		\g@awidth\ps@s\g@awidthmod\ps@s
		\g@atype\ps@s
		pslooparrowoncircle}}

%-----------------------------------------------------------------------------%

\def\ps@deletebox(#1,#2){% width, height in scaled points
\special{"	#1 65536 div
		#2 65536 div
		psdeletebox}}

%-----------------------------------------------------------------------------%

\def\ps@arrowonrectangle(#1,#2) [#3,#4]{% x, y, width, height
\special{"	\ps@convertnum{#1}
		\ps@convertnum{#2}
		\ps@convertnum{#3}
		\ps@convertnum{#4}
		\ps@convertnum{\g@alength}\g@alengthmod\ps@s
		\g@awidth\ps@s\g@awidthmod\ps@s
		\g@atype\ps@s
		[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
		\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
		\g@ldash\ps@s
		psarrowonrectangle}}

%-----------------------------------------------------------------------------%

\def\ps@arrowoncircle(#1,#2) [#3]{% x, y, diameter of circle
\special{"	\ps@convertnum{#1}
		\ps@convertnum{#2}
		\ps@convertnum{#3}
		\ps@convertnum{\g@alength}\g@alengthmod\ps@s
		\g@awidth\ps@s\g@awidthmod\ps@s
		\g@atype\ps@s
		[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
		\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
		\g@ldash\ps@s
		psarrowoncircle}}

%-----------------------------------------------------------------------------%

\def\ps@path(#1,#2)#3{% start coordinates, (xi,yi[,di]) ...
	\def\extractvalues(##1)##2;{%
	  \ifx\endmarker##1\else%
	    \extractvalues##2;\extractvals(##1,0,)%
	  \fi}%
	\def\extractvals(##1,##2,##3,##4){%
	  \ps@convertnum{##1}%
	  \ps@convertnum{##2}%
	  ##3%
	}%
	\special{" mark \extractvalues#3(\endmarker);
			\ps@convertnum{#1}
			\ps@convertnum{#2}
			\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
			[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
			\g@ldash\ps@s
			[ \g@fcolour\ps@s\g@fcolourmod ]\ps@s
			\iffilledareas true \else false\fi\ps@s pspath}}

%-----------------------------------------------------------------------------%

\def\ps@curve#1#2{% base length, (x1,y1,ang1[factor1]) ...
	\def\extractvalues(##1(##2;##3{%
	  \ifx\endmarker##1\else%
	    \extractvalues(##2;{##3}\extractvals(##1[##3,##3];%
	  \fi}%
	\def\extractvals(##1,##2,##3)[##4,##5]##6;{%
	  ##5\ps@s
	  ##4\ps@s
	  ##3\ps@s
	  \ps@convertnum{##2}%
	  \ps@convertnum{##1}%
	}%
	\special{" mark \extractvalues#2(\endmarker(;{#1}
			\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
			[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
			\g@ldash\ps@s
			[ \g@fcolour\ps@s\g@fcolourmod ]\ps@s
			\iffilledareas true \else false\fi\ps@s pscurve}}

%-----------------------------------------------------------------------------%

\def\ps@bubble#1#2{% length factor, (x1,y1) ...
	\def\extractvalues(##1)##2;{%
	  \ifx\endmarker##1\else%
	    \extractvalues##2;\extractvals(##1)%
	  \fi}%
	\def\extractvals(##1,##2){%
	  \ps@convertnum{##2}%
	  \ps@convertnum{##1}%
	}%
	\special{" mark \extractvalues#2(\endmarker);
			#1\ps@s
			\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
			[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
			\g@ldash\ps@s
			[ \g@fcolour\ps@s\g@fcolourmod ]\ps@s
			\iffilledareas true \else false\fi\ps@s psbubble}}

%-----------------------------------------------------------------------------%

\def\ps@dirbowoncircle(#1,#2)(#3,#4,#5)[#6]{% (x1,x2) (y1,y2,d), radius
\special{"	\ps@convertnum{#1}
		\ps@convertnum{#2}
		\ps@convertnum{#3}
		\ps@convertnum{#4}
		#5\ps@s
		\ps@convertnum{#6}
		\ps@convertnum{\g@alength}\g@alengthmod\ps@s
		\g@awidth\ps@s\g@awidthmod\ps@s
		\g@atype\ps@s
		\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
		[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
		\g@ldash\ps@s
		psdirbowoncircle}}

%-----------------------------------------------------------------------------%

\def\ps@dirbowonrectangle(#1,#2)(#3,#4,#5)[#6,#7]{% (x1,x2) (y1,y2,d),
                                                  % xsize, ysize
\special{"	\ps@convertnum{#1}
		\ps@convertnum{#2}
		\ps@convertnum{#3}
		\ps@convertnum{#4}
		#5\ps@s
		\ps@convertnum{#6}
		\ps@convertnum{#7}
		\ps@convertnum{\g@alength}\g@alengthmod\ps@s
		\g@awidth\ps@s\g@awidthmod\ps@s
		\g@atype\ps@s
		\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
		[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
		\g@ldash\ps@s
		psdirbowonrectangle}}

%-----------------------------------------------------------------------------%


